Toward Certification of Machine-Learning Systems for Low Criticality Airborne Applications

The exceptional progress in the field of machine learning (ML) in recent years has attracted a lot of interest in using this technology in aviation. Possible airborne applications of ML include safety-critical functions, which must be developed in compliance with rigorous certification standards of the aviation industry. Current certification standards for the aviation industry were developed prior to the ML renaissance without taking specifics of ML technology into account. There are some fundamental incompatibilities between traditional design assurance approaches and certain aspects of ML-based systems. In this paper, we analyze the current airborne certification standards and show that all objectives of the standards can be achieved for a low-criticality ML-based system if certain assumptions about ML development workflow are applied.

==> notes.tex <==
Restructure: analysis -> proper assumptions

Spelling (EASA, AI - make capital) in the references

\Konstantin{Describe the outline of the table}

6&\Konstantin{ADD 331 OBJECTIVES}
&x&x&x&x&&\\
\hline

\Konstantin{discuss other gaps listed in \cite{eurocae2021SoC}}

\Johann{That is certainly true, but the preprocessing/post-processing of ML (think NN) might very well be parameterized - but that is traditional SW. Do we need to mention that? (not necessarily).}

\Johann{NN architectures are usually parameterized (e.g., number layers, number nodes, but these parameters are design parameters and this not under this objective. right?}

\TODO{put tables in Appendix or inline in the section content (preferable)}

